The MosaicSim Simulator (Full Technical Report)

As Moore's Law has slowed and Dennard Scaling has ended, architects are increasingly turning to heterogeneous parallelism and domain-specific hardware-software co-designs. These trends present new challenges for simulation-based performance assessments that are central to early-stage architectural exploration. Simulators must be lightweight to support rich heterogeneous combinations of general purpose cores and specialized processing units. They must also support agile exploration of hardware-software co-design, i.e. changes in the programming model, compiler, ISA, and specialized hardware. To meet these challenges, we introduce MosaicSim, a lightweight, modular simulator for heterogeneous systems, offering accuracy and agility designed specifically for hardware-software co-design explorations. By integrating the LLVM toolchain, MosaicSim enables efficient modeling of instruction dependencies and flexible additions across the stack. Its modularity also allows the composition and integration of different hardware components. We first demonstrate that MosaicSim captures architectural bottlenecks in applications, and accurately models both scaling trends in a multicore setting and accelerator behavior. We then present two case-studies where MosaicSim enables straightforward design space explorations for emerging systems, i.e. data science application acceleration and heterogeneous parallel architectures.

==> txt/designquestions.tex <==
\section{Crosstalk Characterization and Mitigation: Design Questions}
\subsection{Crosstalk Effects}
In superconducting systems, crosstalk occurs because of two reasons. First, to enable two-qubit operations, qubits are connected to each other using resonators. In Figure \ref{fig:qubit_layout}, each CNOT gate (edges) corresponds to a resonator in hardware. These resonators create an always-on coupling between pairs of qubits. When a control pulse is driven on one of the qubits, the resonator can propagate an unwanted drive to neighboring qubits and corrupt their state. Second, CNOT gates are performed by driving the control qubit at the resonant (0 to 1 transition) frequency of the second qubit. If multiple nearest neighbor or next nearest neighbor qubits have overlapping resonant frequencies, driving a qubit can lead to unwanted state transitions on other qubits.

Although hardware is meticulously engineered to avoid crosstalk by tuning the resonator coupling strengths, using noise cancelling pulse sequences \cite{} and choosing appropriate qubit frequencies \cite{hexagon_paper_cross}, crosstalk effects are still present.
\cite{robin_xtalk} and \cite{flammia_wallman_xtalk} detected crosstalk noise in IBM's 14-qubit system, even when operations are performed on qubits which are separated by multiple hops. Similar effects are present in superconducting systems from other vendors as well \cite{google_xtalk, princeton_xtalk}. These crosstalk effects can significantly impact programs; they can corrupt the quantum state when multiple instructions are executed in parallel. 

Characterizing the effect of such interference is important for designing software techniques to mitigate noise. Since QC systems have highly variable noise properties including variations in gate error rates and coherence times \cite{}, it is important to accurately and frequently measure crosstalk effects across all qubits in a device. This is challenging because crosstalk characterization typically requires extensive quantum compute time to perform a large number of pairwise experiments. Therefore, we ask:

{\em How can we quantify crosstalk errors between two parallel operations? How can we perform such characterization experiments efficiently across the full device? Can we exploit the physical properties of the device to reduce the number of experiments?} 

From the perspective of understanding the implications of crosstalk for programs and compilation, we study: 

{\em How does crosstalk from a gate propagate across the device? Are the effects restricted to a small number of hops around a gate? Is it important to characterize crosstalk for both single and two-qubit gates or is it sufficient to focus only on the latter? And how does crosstalk data change over time?}

\subsection{Crosstalk Mitigation through Instruction Scheduling}
Our experiments on \numdevices\ 20-qubit systems shows that crosstalk between parallel CNOT gates can reduce worsen the error rates up to 11x. When the compiler schedules such operations in parallel, the likelihood of correct execution is drastically reduced. 

To avoid crosstalk a compiler can choose to serialize the interfering operations. However, serialization is expensive on QC systems. Quantum states lose coherence exponentially with time. On IBM systems, coherence times on individual qubits range from 10-100 microseconds --- when a program executes for 50 microseconds on the best qubit with 100us coherence, it is 60\% likely that the state is corrupted. To mitigate this dramatic loss in reliability from decoherence, current compilers such IBM's Qiskit, Riggeti's Quil and TriQ parallelize operations as much as possible. We ask:
 
 {\em How can a compiler optimize the two conflicting objectives of serializing instructions to avoid high crosstalk and parallelizing instructions to avoid decoherence? How much does crosstalk-adaptivity matter for parallel operations on superconducting devices?}


%To measure the loss of coherence, IBM performs characterization experiments on their qubits as part of daily calibration and post the data publicly \cite{}. For each qubit coherence is measured using two metrics: amplitude decay using T1 and and phase decay using T2 time. The T1 time of a qubit is computed by initializing a qubit in the $\ket{1}$ state and measuring the time taken for the state to decay to $\ket{0}$. The T2 time is computed by initializing the state to a uniform superposition of $\ket{0}$ and $\ket{1}$ and measuring when the state loses superposition and decays to either $\ket{0}$ or $\ket{1}$. T1 and T2 times range from X-Y microseconds, average Z microseconds. Figure \ref{} shows the error rates from amplitude decay for two qubits. Since average CNOT gate times are X nanoseconds, losses from decoherence can be significant on qubits which low coherence time. 


%Another question is: Can crosstalk-adaptivity be exploited even with only coarse grained control of timing using barriers at the gate level? 

